dEchorate: a Calibrated Room Impulse Response Database for Echo-aware Signal Processing

This paper presents dEchorate: a new database of measured multichannel Room Impulse Responses (RIRs) including annotations of early echo timings and 3D positions of microphones, real sources and image sources under different wall configurations in a cuboid room. These data provide a tool for benchmarking recent methods in echo-aware speech enhancement, room geometry estimation, RIR estimation, acoustic echo retrieval, microphone calibration, echo labeling and reflectors estimation. The database is accompanied with software utilities to easily access, manipulate and visualize the data as well as baseline methods for echo-related tasks.

==> table_dechorate_db.tex <==
\begin{tabular}{llrrrlrrrrrrrrr}
    \toprule
    Index &            filename &     src & mic & room  &  floor  & ceil & $\cdots$ & signal &   src\_x &  src\_y &  src\_z &  mic\_x &  mic\_y &  mic\_z\\
    \midrule
    {} &  {} &     {} & {} &   {} &   {}         & {}    &  $\cdots$       & {} &   {} &  {} &  {} &  {} &  {} &  {} \\
    217 &  2020-01-22\_22-59-36 &     1 & 0 &   010000 &   0         & 1    &  $\cdots$       & speech &   1.99 &  4.49 &  1.42 &  0.80 &  3.83 &  1.04 \\
    218 &  2020-01-22\_22-59-36 &     1 & 1 &   010000 &   0         & 1    &  $\cdots$       & speech &   1.99 &  4.49 &  1.42 &  0.84 &  3.84 &  1.04 \\
    219 &  2020-01-22\_22-59-36 &     1 & 2 &   010000 &   0         & 1    &  $\cdots$       & speech &   1.99 &  4.49 &  1.42 &  0.88 &  3.86 &  1.04 \\
    220 &  2020-01-22\_22-59-36 &     1 & 4 &   010000 &   0         & 1    &  $\cdots$       & speech &   1.99 &  4.49 &  1.42 &  0.94 &  3.88 &  1.04 \\
    221 &  2020-01-22\_22-59-36 &     1 & 5 &   010000 &   0         & 1    &  $\cdots$       & speech &   1.99 &  4.49 &  1.42 &  1.04 &  3.91 &  1.04 \\
    {} &  {} &     {} & {} &   {} &   {}         & {}    &  $\cdots$       & {} &   {} &  {} &  {} &  {} &  {} &  {} \\
    \bottomrule
\end{tabular}

==> table_results_mds.tex <==
\begin{table}[]
\centering
\caption{\label{tab:res_mds} Mismatch between geometric measurements and signal measurements in terms of maximum (Max.), average (Avg.) and standard deviation (Std) of absolute mismatch in centimeters.
The goodness of match (GoM) between the signal and geometrical measurements is reported as the fraction of matching echo timings for different thresholds in milliseconds.}

\begin{tabular}{lllll}
\toprule
& Metrics        & $\bIPS$               & $\dMDS$          & $\dcMDS$          \\
\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\rotatebox{90}{\scriptsize Geom.}}}
&   Max.             & 0            & $6.1$         & $1.07$        \\
&   Avg.$\pm$Std.    & 0            & $1.8\pm1.4$    & $0.39\pm0.2$  \\
% \rule{0pt}{0.05em}\\
\midrule
\multicolumn{1}{c}{\multirow{2}{*}{\rotatebox{90}{\scriptsize Signal}}}
&   Max.          & $5.86$         & $1.20$         & $1.86$       \\
&   Avg.$\pm$Std. & $1.85\pm 1.5$  & $0.16\pm0.2$   & $0.41\pm0.3$ \\
% \rule{0pt}{0.05em}\\
\midrule
\multicolumn{1}{c}{\multirow{3}{*}{\rotatebox{90}{\scriptsize Mismatch}}}
&  GoM (1.0 ms)   & $97.9 \%$      & $93.4 \%$      & $98.1 \%$ \\
&  GoM (0.1 ms)   & $26.6 \%$      & $44.8 \%$      & $53.1 \%$ \\
&  GoM (0.05 ms)  & $12.5 \%$      & $14.4 \%$      & $30.2 \%$ \\
% \rule{0pt}{0.05em}\\
\bottomrule
\end{tabular}
\end{table}
